Lens: A Knowledge-Guided Foundation Model for Network Traffic

Network traffic refers to the amount of data being sent and received over the Internet or any system that connects computers. Analyzing network traffic is vital for security and management, yet remains challenging due to the heterogeneity of plain-text packet headers and encrypted payloads. To capture the latent semantics of traffic, recent studies have adopted Transformer-based pretraining techniques to learn network representations from massive traffic data. However, these methods pre-train on data-driven tasks but overlook network knowledge, such as masking partial digits of the indivisible network port numbers for prediction, thereby limiting semantic understanding. In addition, they struggle to extend classification to new classes during fine-tuning due to the distribution shift. Motivated by these limitations, we propose \Lens, a unified knowledge-guided foundation model for both network traffic classification and generation. In pretraining, we propose a Knowledge-Guided Mask Span Prediction method with textual context for learning knowledge-enriched representations. For extending to new classes in finetuning, we reframe the traffic classification as a closed-ended generation task and introduce context-aware finetuning to adapt to the distribution shift. Evaluation results across various benchmark datasets demonstrate that the proposed Lens~achieves superior performance on both classification and generation tasks. For traffic classification, Lens~outperforms competitive baselines substantially on 8 out of 12 tasks with an average accuracy of \textbf{96.33\%} and extends to novel classes with significantly better performance. For traffic generation, Lens~generates better high-fidelity network traffic for network simulation, gaining up to \textbf{30.46\%} and \textbf{33.3\%} better accuracy and F1 in fuzzing tests. We will open-source the code upon publication.

==> secs/back_intro.tex <==
Network traffic serves as the lifeblood of data exchange in the field of information technology. In order to consolidate network security, streamline the network management process, and ensure the delivery of high-quality network services, it is crucial to delineate the characteristics of the traffic. This can be achieved through the investigation of its latent features and the use of large-scale traffic data. Consequently, two tasks have gained considerable attention in the study of network traffic - traffic understanding \cite{classification} and traffic generation \cite{netshare, first-gan}.

% \shao{We may need to emphasize that our method needs less fine-tune data, high accuracy, and applicable to more downstream tasks.}
Traffic understanding tasks intend to categorize network traffic in multiple aspects: ranging from malware detection to application classification \cite{fingerprint, k-fingerprint, etbert}. These tasks probe into the hidden features embedded in traffic to fulfill their respective goals. Since the characteristics that matter can vary greatly between tasks in network traffic analysis, manual feature extraction from traffic becomes an arduous work with a rather poor degree of generalization. Although existing approaches like \cite{df, fs-net, deeppacket, datanet} circumvent this exhaustive process by leveraging deep learning methods, they remain reliant on a substantial volume of labeled data for model training, limiting their flexibility to adapt to new tasks. Concurrently, to alleviate the lack of data in some scenarios, network traffic generation enhances the pool of network traffic by developing methods to synthesize artificial header traces. However, these methods like \cite{ns-3, first-gan, netshare} can be either difficult to tailor for various downstream tasks or expensive when it comes to training a customized model.

% \ziyu{The first few sentences are a bit hard to follow. "Furthermore, shares..." is missing a subject.}
% \shao{To overcome the above issues, recent works mainly adopt pre-training methods to }
To address the identified challenges, recent methodologies leverage pre-training techniques. Pre-training methods like \cite{bert, t5, gpt3} utilize a vast corpus of unlabeled data to understand corpus patterns, relying on a small amount of labeled data for deploying models in specific applications. Considering the similarities between network traffic and natural language, which both present as sequences of strings, new models like PERT \cite{pert} and ET-BERT \cite{etbert} have been created for traffic analysis. However, despite their proficiency in understanding encrypted traffic, BERT-based models \cite{bert} lack generative capabilities due to their encoder-only architecture. Indeed, GPT-based models \cite{gpt, gpt2, gpt3} are well-regarded for their generation abilities. However, they learn from previous information in a sequence without considering the following information. This unidirectional learning approach falls short for network traffic analysis since they do not account for the global context of input string, where the order of header fields is not pivotal, for example, packet length focuses on the global context information.  Therefore, an integrated encoder-decoder architecture is suggested as a more comprehensive solution for the issues earlier mentioned.

% \ziyu{1. Is there a better name than "Lens"? It does not sound obvious to be about "network". How about NetT5 (similar to CodeT5)? 2. Table 1 is not referred to anywhere. It actually provides a clear summary of our contribution. 3. Still about table 1: (a) "Anonymize" is not clear to me and is not discussed in Intro either; (b) The categories can be made more clear to include Architecture (Tok, Enc, Dec), Pre-training (w or w/o curated objective functions, Anonymization), and Supporting Tasks (Understanding, Generation).}
In this paper, we present Lens, a pioneering model utilizing the T5 architecture \cite{t5, codet5} as the underlying framework for analyzing network traffic. We categorize network tasks into two primary types: understanding tasks, and generation tasks focusing on header synthesis. The choice of T5 over models like GPT is deliberate. T5's sequence-to-sequence denoising pre-training is better suited for handling both understanding and generation tasks in network contexts. It excels because network traffic, often characterized by diverse and complex data streams, necessitates a model capable of processing input data effectively. Unlike GPT's decoder-only approach, T5's encoder-decoder structure better manages this complexity, making it an ideal pick for network traffic analysis. Extensive tests have confirmed its effectiveness.


Our proposed framework consists of three stages: tokenization, pre-training, and fine-tuning. Considering that network protocols vary and payload data may be encrypted or unencrypted, Lens standardizes these different traffic types by converting all traffic content into a hexadecimal format at the tokenization stage. To further investigate the best configuration to train a tokenizer, we explore the uses of SentencePiece and WordPiece algorithms with different vocabulary sizes. The pre-training process involves utilizing three tasks - Masked Span Prediction (MSP), Packet Order Prediction (POP), and Homologous Traffic Prediction (HTP) to enable Lens to discern latent patterns inherent in network traffic. MSP serves as a denoising task that prompts Lens to recover masked tokens, thereby enabling the model to capture representations within the network traffic. Meanwhile, POP predicts the order of packets within a singular traffic input, facilitating the capture of latent data features within the same session flow. Meanwhile, inspired by \cite{etbert}, HTP aids in pinpointing relational patterns across different flows. During the fine-tuning stage, we utilize task-oriented prompts coupled with a minimal amount of task-specific labeled data to delicately adjust the parameters of the Lens, which empowers the Lens with the ability to effectively adapt to various understanding and generation downstream tasks compared with previous works.

The main contributions of our work can be summarized as follows: (1) We introduce Lens, the first network traffic model using the T5 architecture, designed to handle both understanding and generating network traffic tasks by leveraging large amount of unlabeled traffic data. (2) We explore various tokenization algorithms and analyze how different settings affect network traffic that has been transformed into hexadecimal format. Our findings show that the WordPiece algorithm outperforms the SentencePiece, and further enhancement in pre-training performance is observed with the use of predefined vocabulary. (3) We incorporate three distinct tasks into the model's pre-training stage, namely Masked Span Prediction (MSP), Packet Order Prediction (POP), and Homologous Traffic Prediction (HTP). Within this framework, MSP functions as an encoder-decoder task for efficiently capturing traffic representations, whereas POP and HTP, operating as encoder-only tasks, capture intrinsic patterns and discern the relationships among different traffic flows respectively. (4) We evaluate Lens on understanding and generation tasks across 6 real-world datasets \cite{vpn, tor, ustc, cp, doh, iot} among 15 understanding tasks and 5 header fields generation tasks, using 50\% $\sim$ 95\% less labeled data for fine-tuning compared to ET-BERT. Our extensive experimentation demonstrates that Lens outperforms  existing state-of-the-art methods by improving flow-level traffic understanding accuracy to 96.15\% (10.75\%$\uparrow$), packet-level traffic understanding accuracy to 97.56\% (0.59\%$\uparrow$) on average, and decreasing the traffic generation JSD to 0.0498 (0.1353$\downarrow$) and the TVD to 0.0825 (0.3548$\downarrow$) on average, showcasing its impressive generalization capability.
% \begin{enumerate}[itemsep=3pt,topsep=0pt,parsep=0pt, leftmargin=13pt]
%     \item We introduce Lens, the first network traffic model using the T5 architecture, designed to handle both understanding and generating network traffic tasks by leveraging large amount of unlabeled traffic data.
%     \item We explore various tokenization algorithms and analyze how different settings affect network traffic that has been transformed into hexadecimal format. Our findings show that the WordPiece algorithm outperforms the SentencePiece, and further enhancement in pre-training performance is observed with the use of predefined vocabulary.
%     \item We incorporate three distinct tasks into the model's pre-training stage, namely Masked Span Prediction (MSP), Packet Order Prediction (POP), and Homologous Traffic Prediction (HTP). Within this framework, MSP functions as an encoder-decoder task for efficiently capturing traffic representations, whereas POP and HTP, operating as encoder-only tasks, capture intrinsic patterns and discern the relationships among different traffic flows respectively.
%     \item We evaluate Lens on understanding and generation tasks across 6 real-world datasets \cite{vpn, tor, ustc, cp, doh, iot} among 15 understanding tasks and 5 header fields generation tasks, using 50\% \~ 95\% less labeled data for fine-tuning compared to ET-BERT. Our extensive experimentation demonstrates that Lens outperforms  existing state-of-the-art methods by improving flow-level traffic understanding accuracy to 96.15\% (10.75\%$\uparrow$), packet-level traffic understanding accuracy to 97.56\% (0.59\%$\uparrow$) on average, and decreasing the traffic generation JSD to 0.0498 (0.1353$\downarrow$) and the TVD to 0.0825 (0.3548$\downarrow$) on average, showcasing its impressive generalization capability.
% \end{enumerate}

% \ziyu{Before related work, consider adding a "Background" section to present some of the terminologies in network research. Qineng, you may recall how much time you spent on explaining "packets", "flow", etc., when you presented your progress to me. I assume that most KDD reviewers do not have this background. You could also use this section to educate people about the significance of modeling network traffic (e.g., connecting to cyber threat detection, etc.).}
\section{Background Knowledge}
In the realm of cybersecurity and network management, network traffic is indispensable for monitoring, detecting, and preventing malicious activities, ensuring efficient data flow and optimizing performance. A pcap (Packet Capture) file represents a recorded packet traffic on a network segment, capturing data as it traverses the electronic corridors, aiding forensic analysis and network diagnostics. It encapsulates the concept of one or more session flows, which are a series of related packet exchanges between two endpoints, providing context for communication patterns and potential threats. A packet, the fundamental unit of data transmitted over a network, encapsulates user and control information crucial for delivering data to its intended destination. Pre-training approaches like GPT, T5, and BERT provide robust foundations for multi-task transfer learning by comprehending extensive, unlabeled datasets and fostering adaptable models tuned with less data for domain-specific tasks, yielding significant applications in versatile network scenarios.


In this paper, we present Lens, a pioneering model utilizing the T5 architecture \cite{t5, codet5} as the underlying framework for analyzing network traffic. We categorize network tasks into two primary types: understanding tasks, involving classification, and generation tasks, focusing on header synthesis. The choice of T5 over models like GPT, which primarily focuses on decoding, is deliberate. T5's sequence-to-sequence denoising pre-training is better suited for handling both understanding and generation tasks in network contexts. This design choice is particularly advantageous because network traffic, often characterized by diverse and complex data streams, necessitates a model capable of processing input data effectively. T5's encoding-decoding structure, unlike GPT's decoding-only 

T5's encoding-decoding structure, unlike GPT's decoding-only approach, allows for more nuanced handling of these varied inputs, making it an ideal choice for the multifaceted demands of network traffic analysis. This suitability has been reinforced by comprehensive empirical testing.

